When does the student surpass the teacher? Federated Semi-supervised Learning with Teacher-Student EMA

Semi-Supervised Learning (SSL) has received extensive attention in the domain of computer vision, leading to development of promising approaches such as FixMatch. In scenarios where training data is decentralized and resides on client devices, SSL must be integrated with privacy-aware training techniques such as Federated Learning. We consider the problem of federated image classification and study the performance and privacy challenges with existing federated SSL (FSSL) approaches. Firstly, we note that even state-of-the-art FSSL algorithms can trivially compromise client privacy and other real-world constraints such as client statelessness and communication cost. Secondly, we observe that it is challenging to integrate EMA (Exponential Moving Average) updates into the federated setting, which comes at a trade-off between performance and communication cost. We propose a novel approach FedSwitch, that improves privacy as well as generalization performance through Exponential Moving Average (EMA) updates. FedSwitch utilizes a federated semi-supervised teacher-student EMA framework with two features - local teacher adaptation and adaptive switching between teacher and student for pseudo-label generation. Our proposed approach outperforms the state-of-the-art on federated image classification, can be adapted to real-world constraints, and achieves good generalization performance with minimal communication cost overhead.

==> tables/cifar_10_res.tex <==
\begin{table*}[htbp] \label{cifar10-results}
\caption{Performance of all competing approaches on the CIFAR-10 dataset. For each approach, we report the mean performance, along with standard deviation over five trials and 800 epochs. The best configuration for each approach is obtained through a hyper-parameter search. Results are reported for both Batch-IID and Batch-NonIID settings under labels-at-client and labels-at-server configurations.* refers to existing work that cuts off training at 200 rounds when not yet fully converged.}
\centering
\begin{tabular}{c|cccc}
\hline
                 & \multicolumn{4}{c}{Client/Server Configuration}   \\ \hline
Approach         & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} \\ Labels at Client\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}LaS (Sequential, Parallel)\\ (Labels at Server)\end{tabular}} \\ \hline
                 & Batch-IID                        & Batch-NonIID                                       & Batch-IID                               & Batch-NonIID                               \\ \hline
FedRGD           &  71.61      &     69.05                                               &        63.32                                 &                   63.24                         \\
FedMatch*         &  52.13$\pm$0.34                                &             52.25$\pm$0.81                                    &           44.95$\pm$0.49                              &                  44.17$\pm$0.19                          \\
FedProx-FixMatch* &   47.20 $\pm$ 0.12                               &             45.55 $\pm$ 0.63                                    &      25.61$\pm$0.32                                  &        9.21$\pm$0.24                                   \\
FedProx-FixMatch (ours) &   90.02$\pm$0.4                               &               89.54$\pm$0.82                                     &      (89.8$\pm$0.72, \textbf{87.85$\pm$0.9})                                   &        (88.19$\pm$1.10, \textbf{87.28$\pm$0.79})                                  \\
\vanillaema          &  89.43$\pm$0.60                                &       85.43$\pm$0.87                                             &      (89.15$\pm$0.95, 87.34$\pm$0.77)                                   &     (73.26$\pm$0.98, 72.08$\pm$1.89)                               \\
% \vanillaema [lo] & 89.35$\pm$1.318  & 84$\pm$1.01 & 88.67$\pm$0.90;86.68$\pm$0.93 & 75.74$\pm$1.64;75.63$\pm$0.889 \\
\freqema &  89.94$\pm$0.91                               &     87.41$\pm$0.61                                               &  (89.29$\pm$0.63, 89.12$\pm$0.46)                                 &                 (78.43$\pm$1.63, 77.68$\pm$1.03)                          \\
% \freqema [lo] & 88.96$\pm$1.04 & 87.52$\pm$1.21 & 89.43$\pm$0.45;90.02$\pm$0.47 & 85.08$\pm$0.38;86.15$\pm$0.95 \\
\proposedregmethod  &  \textbf{90.24$\pm$0.60 }                               &     \textbf{89.57$\pm$0.55 }                                             &  (\textbf{90.22$\pm$0.49}, 87.84$\pm$0.63)                                       &                 (\textbf{88.91$\pm$0.50}, 87.04$\pm$0.68)                       \\
\hline
\end{tabular}
\end{table*}

==> tables/fmnist_res.tex <==
\begin{table}[tbp] \label{fashion-mnist-results}
\caption{Performance of all competing approaches on the Fashion-MNIST dataset. For each approach, we report the mean performance, along with standard deviation over five trials and 800 epochs. The best configuration for each approach is obtained through a hyper-parameter search. Results are reported for the Streaming-NonIID settings under both labels-at-client and labels-at-server configurations.}
\centering
\setlength\tabcolsep{1.5pt}
\begin{tabular}{c|cc}
\hline
                 & \multicolumn{2}{c}{Client/Server Configuration} \\ \hline
Approach         & \begin{tabular}[c]{@{}c@{}} \\ Labels at Client\end{tabular} & \begin{tabular}[c]{@{}c@{}}Labels at Serve\\ (Seq, Par) \end{tabular} \\ \hline
                 & Streaming-NonIID       & Streaming-NonIID       \\ \hline
FedMatch         & 77.95$\pm$0.14                     & \textbf{84.15$\pm$0.31}                     \\ \hline
FedProx-FixMatch(o) & 86.51$\pm$1.05 & \begin{tabular}[c]{@{}c@{}} 82.77$\pm$1.04 \\ 80.92$\pm$2.68 \end{tabular}                    \\
FedProx-FixMatch & 62.40$\pm$0.43 & 73.71$\pm$0.32 \\
\vanillaema           &          82.70$\pm$0.67       &         \begin{tabular}[c]{@{}c@{}} 77.49$\pm$5.66 \\ 76.04$\pm$4.57 \end{tabular}             \\
\proposedregmethod           & \textbf{88.94$\pm$0.52}                     & \begin{tabular}[c]{@{}c@{}} 81.72$\pm$2.48 \\ 82.85$\pm$1.27 \end{tabular}                   \\
\freqema  & 86.48$\pm$0.98                    & \begin{tabular}[c]{@{}c@{}} 81.15$\pm$3.93 \\ 76.64$\pm$4.38 \end{tabular}                       \\ \hline
\end{tabular}
\end{table}
